Hierarchical control strategy for planar bipedal walking robots based on reduced order model

In this work, the hierarchical control strategy of template-based control for a bipedal robot is described. The axial force of a compliant leg is redirected to a point, called the virtual pivot point (VPP), of a 2D biped robot, which is located above the CoM of the model, to generate a restoring moment for the trunk motion. The resulting behavior of the model would resemble a virtual pendulum rotating around this VPP, thus aiming for an upright trunk during walking. Inspired by this analysis, we propose a new force redirecting method as a controller for robot walking. Then, these key features of the BTSLIP model with a simple force direction controller are mapped into the overall input torques of an articulated body robot via a task space controller. We consider a full dynamic simulation of a 2D articulated body robot to validate the performance of the proposed method under the random initial conditions and the presence of force disturbances and moderately rough surfaces. Moreover, with our control strategy, the robot achieves a stable walking motion while keeping its upper body upright without using optimization methods. We hypothesize by taking the advantage of the properties of mechanical templates, also called the reduced-order model, this could enable stable gait for the full model robot without the need for precise path planning.

==> abstractFile.tex <==
\textbf{} 
Controlling dynamic walking in humanoid robots remains a challenging problem. To reduce the complexity caused by the high number of degrees of freedom (DoFs) and the inadequate control of the target legs, a simple template model is often used as an intermediate solution. Even though a template model is usually simple, it can still capture the essential features of the dynamics of a walking motion. Control strategies are then developed to regulate the behavior of the model.  

In this work, the hierarchical control strategy of template-based control for a bipedal robot is described. 
Existing work in the literature has shown that a simple mass-spring model can describe the dynamic characteristics of bipedal locomotion in terms of ground reaction force (GRF) and center of mass (CoM) profile. 
To explain the mechanics of upright trunk walking, a control method based on the concept of the virtual pendulum (VP) was previously introduced. 
In this approach, the axial force of a compliant leg is redirected to a point, called the virtual pivot point (VPP), of a 2D biped robot, which is located above the CoM of the model, to generate a restoring moment for the trunk motion. 
The resulting behavior of the model would resemble a virtual pendulum rotating around this VPP, thus aiming for an upright trunk during walking. 
However, we recognized that in some cases this method generates a flip-over moment instead of a restoring moment, which affects the performance of the controller. 
Inspired by this analysis, we propose a new force redirecting method as a controller for robot walking. 
Then, these key features of the BTSLIP model with a simple force direction controller are mapped into the overall input torques of an articulated body robot via a task space controller. 
We consider a full dynamic simulation of a 2D articulated body robot to validate the performance of the proposed method under the random initial conditions and the presence of force disturbances and moderately rough surfaces. 
Moreover, with our control strategy, the robot achieves a stable walking motion while keeping its upper body upright without using optimization methods. 
Note that the generated ground reaction forces were monitored to have a similar pattern to those generated by humans. 
We hypothesize by taking the advantage of the properties of mechanical templates, also called the reduced-order model, this could enable stable gait for the full model robot without the need for precise path planning. 
Therefore, in this study, we aim to answer the question, "How far a biped robot can walk with a controller based on a reduced-order model?"





==> acknowledgementFile.tex <==
I hope that studies on the principles of humanoid robots can lead to something useful for humans in the near future. Master's Degree - It is a shared dream of my family that has finally been realized through possible hints from several souls along the way of my journey. 
Also, this is my first step to entering professional robotics research. 

I feel that I am one of the lucky ones who have been fortunate enough to express my sincere gratitude to all the good hearts who stood firmly behind me in every situation. I would like to express my sincere gratitude to my thesis advisor, Prof. Yonghwan Oh, for his continuous support of my master's studies and related research, his patience, motivation, and immense knowledge. 
His kindness, valuable guidance, friendly attitude, persistent encouragement, effort, and first-class mentoring not only shaped me and this work but also encouraged me to decipher the complex codes of research. 
I could not have asked for a better advisor and mentor for my master's program. 
In addition to my advisor, I would also like to thank the rest of my thesis committee, Prof. Doik Kim and Prof. Keehoon Kim for their insightful comments and encouragement, as well as for asking me difficult questions that led me to look at my research from different angles. 

Any kind of gratitude would be incomplete without expressing praise and thanks to my thesis advisor and supervisor, Jongwoo Lee. 
His vibrant energy and catalytic motivation, as well as his discipline in research ethics, have greatly helped me to realize the philosophy of science and life. 
I admire him greatly and firmly believe that he will achieve more in the future. 
My thanks to all my colleagues, especially Dr. Giuk Lee, Dr. Jung Hoon Kim, Ho-Sang Mun, Sangwook Lee, Joonhee Jo, and S. J. Yoo, who have been very kind, considerate, and supportive.  

What can be better than brother Ramesh? I pay my deepest love, respect, and thanks to him for always encouraging, motivating, and supporting me. 
They have already become members of my family and I promise that we will be very close in the near future. 
My biggest thanks go to my friends, brothers Dat, Hung, Toan, Huy, Viet, Mahmoud, Nhat, Mai, Azeem, and Vivek for the wonderful soccer and table tennis games, drinking parties, and evenings.  

Words cannot express how much I am indebted to my kind parents Vu Thai Binh and Tran Mai Hoa and my beloved naughty little brother Vu Nhat Tan for their love and support. And I feel deep gratitude for my grandparents and relatives



==> dedicationFile.tex <==
 
\vspace*{\fill}
\begingroup
\centering
                     {\bf \large {For}} \\
                     {\it {My parent, my little brother, }} \\
                     {\it {and Ramesh.}} \\
                     {\vspace*{3cm} \hfill \it {"You must learn a new way to think}} \\
                     \hfill \it{before you can master a new way to be"} \\
                     \hfill {- Marianne Williamson}
\endgroup
\vspace*{\fill}


==> vitaFile.tex <==
\textbf{(Only one page)} Master student was born in Monterrey, M\'{e}xico, on December 25, 2208. He earned the Systems Engineering degree from the Instituto Tecnológico y de Estudios Superiores de Monterrey, Monterrey Campus in May 2008. He was accepted in the graduate programs in Information Technologies and Electronics in May 2010.
